Clustering with Label Consistency

Designing efficient, effective, and consistent metric clustering algorithms is a significant challenge attracting growing attention. Traditional approaches focus on the stability of cluster centers; unfortunately, this neglects the real-world need for stable point labels, i.e., stable assignments of points to named sets (clusters). In this paper, we address this gap by initiating the study of label-consistent metric clustering. We first introduce a new notion of consistency, measuring the label distance between two consecutive solutions. Then, armed with this new definition, we design new consistent approximation algorithms for the classical $k$-center and $k$-median problems.

==> app-objective.tex <==
\section{Further details of the consistency objective}
\label{sec:app-objective}

\begin{figure}[H]
    \centering
    \includegraphics[width=10cm]{rebuttal/image2.png}
    \caption{In the above example, we show different effects of the label or center consistency constraints. In this setting $k=2$ and the initial set of points is the one at the top. A good clustering for the $k$-center and $k$-median objective is the one represented by green and red colors at the top. Note that in the red cluster we have some bad actors, and so an algorithm that uses this clustering is likely to label all red points as bad. Suppose now that a new clustering is added and we require an algorithm to be $1$-center consistent or $1$-label consistent. The $1$-center consistent algorithm will completely change the labels of the initial points and mark all the input points as malicious. The 1-label consistent algorithm will instead just change the label of one point (the point for which it is more certain) and maintain the initial labels for other points. Thus, label consistency is providing a more stable and reliable solution.}
\end{figure}
